Evaluation of RANS-based turbulence models for isothermal flow in a realistic can-type gas turbine combustor application

The present study assesses RANS-based turbulence models to simulate isothermal flow in a combustor representing a constituent can combustor of can-annular configuration used in jet engines. Two-equation models (standard $k-\epsilon$, realizable $k-\epsilon$, standard $k-\omega$, SST $k-\omega$), and Linear Pressure Strain - Reynolds Stress Model (LPS-RSM), are assessed by comparing their predictions of mean axial and transverse velocity, turbulent kinetic energy, and shear stress with the experimental data at the primary and dilution hole planes in combustor. While the two-equation models generally have failed to predict the confined swirling flow at both positions accurately, the SST $k-\omega$ model yielded the most accurate, followed by standard $k-\omega$ and realizable $k-\epsilon$ models. The discrepancies between the computational and experimental results could be attributed to the isotropic turbulence assumptions, which, however, are invalid for confined swirling flows. Further, the two-equation model formulations cannot capture the intricacies of vortex flow and its interaction with the surroundings in confined swirling flows. LPS-RSM, which considers turbulence anisotropy, showed some promise, although overpredicted results follow the trend with experimental values at the primary holes plane. However, at dilution holes plane, the model overpredicted the velocity field and underestimated turbulence field, including turbulent kinetic energy and shear stress. These observed discrepancies can be ascribed to the pressure-strain correlation in the LPS-RSM, which assumes the pressure is a linear function of the strain-rate tensor. However, for complex flows, this linear assumption is quite simplistic. Hence, this study suggests that more advanced turbulence models such as non-LPS-RSM are needed to accurately predict the confined swirling flow in combustors.

==> Makefile <==
# type "make" command in Unix to create ps and pdf file 
#
#Colors
gray=\e[1;30m
red=\e[0;31m
RED=\e[1;31m
blue=\e[0;34m
BLUE=\e[1;34m
green=\e[0;32m
GREEN=\e[1;32m
cyan=\e[0;36m
CYAN=\e[1;36m
NC=\e[0m # No Color

# the documents to be compiled by default
# set defaultfile to the name of the main file without the .tex
#
defaultfile = $(foreach i,$(filter-out ,$(shell grep -l documentclass *.tex)), $(basename $i))
#
ASPELL = aspell -t -c --mode=tex
ISPELL = ispell -t  --mode=tex
LATEX = latex -interaction=batchmode
BIBTEX = bibtex 
MAKEINDEX = makeindex
PDFLATEX = pdflatex -interaction=batchmode
#
DVIPS = dvips -Pwww
DVIPDF = dvipdf 
PSPDF = ps2pdf
#
all: pdf clean
#
pdf:
	@echo -e ""
	@echo -e "$(BLUE)====> Default file being compiled: $(RED)$(defaultfile).tex$(NC)"
	@echo -e ""
	@echo -e "$(BLUE)====> $(green)Running LaTeX$(NC)" ;
	$(LATEX) $< $(QUIET)$(defaultfile)
#
#	@echo -e "$(BLUE)====> $(green)Running PDFLaTeX to generate PDF document$(NC)" ;
#	$(PDFLATEX) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Running BibTex$(NC)" ;
	$(BIBTEX) $< $(QUIET)$(defaultfile)
#	
#	@echo -e "$(BLUE)====> $(green)Running aspell$(NC)" ;
#	$(ASPELL) $< $(QUIET)$(defaultfile).tex
#
#	@echo -e "$(BLUE)====> $(green)Running ispell$(NC)" ;
#	$(ISPELL) $< $(QUIET)$(defaultfile).tex
#
	@echo -e "$(BLUE)====> $(green)Running Makeindex$(NC)" ;
	$(MAKEINDEX) $< $(QUIET)$(defaultfile).nlo -s nomencl.ist -o  $(QUIET)$(defaultfile).nls
#
#	@echo -e "$(BLUE)====> $(green)Running PDFLaTeX to generate PDF document$(NC)" ;
#	$(PDFLATEX) $< $(QUIET)$(defaultfile)
#
#	@echo -e "$(BLUE)====> $(green)Running PDFLaTeX to generate PDF document$(NC)" ;
#	$(PDFLATEX) $< $(QUIET)$(defaultfile)
#
#
	@echo -e "$(BLUE)====> $(green)Running LaTeX$(NC)" ;
	$(LATEX) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Running LaTeX$(NC)" ;
	$(LATEX) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Generating PS document from DVI document$(NC)" ;
	$(DVIPS) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Generating PDF document from DVI document$(NC)" ;
	$(DVIPDF) $< $(QUIET)$(defaultfile)
#
#	@echo -e "$(BLUE)====> $(green)Generating PDF document from PS document$(NC)" ;
#	$(PSPDF) $(defaultfile).ps $(defaultfile).pdf
#
clean:
	@echo -e "$(RED)====> $(red)Cleaning up temporary files$(NC)"
	rm -f *.brf *.glo *.ist *.nlo  *.out *.spl *.log *.aux *.*% *.lof *.gls *.nls
	rm -f *.lop *.lot *.toc *.idx *.ilg *.ind *.bbl *.blg *.backup *.bak *~




==> nomenclature.tex <==
\fontsize{10}{10pt}\selectfont
%
 \nomenclature[g0]{\textit{Greek letters}}{}
 \nomenclature[d0]{\textit{Dimensionless groups}}{}
 \nomenclature[s0]{\textit{Subscripts and Superscripts}}{}
 \nomenclature[z0]{\textit{Abbreviations}}{}
%
%%%%%%%%%%% Abbreviations
\nomenclature[zcfd]{CFD}{computational fluid dynamics}
\nomenclature[zedl]{EDL}{electrical double layer}
\nomenclature[zeve]{EVE}{electroviscous effect}
\nomenclature[zevf]{EVF}{electroviscous flow}
\nomenclature[zfem]{FEM}{finite element method}
\nomenclature[zfvm]{FVM}{finite volume method}
\nomenclature[zpdes]{PDEs}{partial differential equations}
\nomenclature[zpdps]{PDF}{pressure-driven flow}
\nomenclature[zsaes]{SAEs}{simultaneous algebraic equations}
%
%%%%%%%%%%% List of Symbols
%\nomenclature[aB]{$B$}{charge-dependent slip length (\eqn\ref{eq:26}), --}
%\nomenclature[ab]{$b$}{charge-dependent slip length (\eqn\ref{eq:20}), m}
%\nomenclature[aB0]{$B_\text{0}$}{slip length (\eqn\ref{eq:26}), --}
%\nomenclature[ab0]{$b_\text{0}$}{slip length (\eqn\ref{eq:20}), m}
%\nomenclature[aD]{$\mathcal{D}$}{diffusivity of the positive and negative ions, assumed equal ($\mathcal{D}_{+}=\mathcal{D}_{-}=\mathcal{D}$), m$^2$/s}
%\nomenclature[ad]{$d$}{equilibrium distance of Lennard-Jones potential ($=0.4\times 10^{-9}$,  \eqn\ref{eq:20}), m}
\nomenclature[adc]{$d_{\text{c}}$}{contraction ratio ($=W_{\text{c}}/W$), --}
\nomenclature[aDj]{$\mathcal{D}_{j}$}{diffusivity of the ions of type j, assumed equal ($\mathcal{D}_{+}=\mathcal{D}_{-}=\mathcal{D}$), m$^2$/s}
\nomenclature[ae]{$e$}{elementary charge of a proton ($=1.602176634\times 10^{-19}$), C or A.s}
\nomenclature[aE]{$E_{\text{x}}$}{induced electric field strength ($=-\partial U/\partial x$), V/m or --}
\nomenclature[afj]{$\mathbf{f_\text{j}}$}{flux density of the ions of type j (\eqn\ref{eq:9}), 1/(m$^2$.s)}
\nomenclature[aIc]{$I_{\text{c}}$}{conduction current density (\eqn\ref{eq:7}), A/m$^2$ or --}
\nomenclature[aId]{$I_{\text{d}}$}{diffusion current density (\eqn\ref{eq:7}), A/m$^2$ or --}
\nomenclature[aIs]{$I_{\text{s}}$}{streaming current density (\eqn\ref{eq:7}), A/m$^2$ or --}
\nomenclature[akB]{$k_{\text{B}}$}{Boltzmann constant ($=1.380649\times 10^{-23}$), J/K}
%\nomenclature[alB]{$l_\text{B}$}{Bjerrum length ($=0.7\times 10^{-9}$, \eqn\ref{eq:20}), m}
\nomenclature[aLc]{$L_{\text{c}}$}{length of contraction section, m or --}
\nomenclature[aLd]{$L_{\text{d}}$}{length of downstream outlet section, m or --}
\nomenclature[aLu]{$L_{\text{u}}$}{length of upstream inlet section, m or --}
\nomenclature[an+]{$n_{+}$}{local number density of positive ions (\eqn\ref{eq:6}), 1/m$^3$ or --}
\nomenclature[an-]{$n_{-}$}{local number density of negative ions (\eqn\ref{eq:6}), 1/m$^3$ or --}
\nomenclature[an0]{$n_{0}$}{bulk density of the ions of type j, 1/m$^3$}
\nomenclature[anj]{$n_{j}$}{local number density of the ions of type j, 1/m$^3$}
\nomenclature[ans]{$n^*$}{excess charge ($=n_{+}-n_{-}$), 1/m$^3$ or --}
\nomenclature[ant]{$n^{**}$}{normalized excess charge,  --}
\nomenclature[aP]{$P$}{pressure, Pa or --}
\nomenclature[aT]{$T$}{temperature, K}
\nomenclature[aU]{$U$}{total electrical potential, V or --}
\nomenclature[aU]{$U_{\text{c}}$}{characteristic total electrical potential, V}
\nomenclature[aV]{$\mathbf{V}$}{velocity vector, m/s or --}
\nomenclature[aVa]{$\overline{V}$}{average velocity of the fluid at the inlet, m/s}
\nomenclature[aVx]{$V_x$}{x-component of the velocity, m/s or --}
\nomenclature[aVy]{$V_y$}{y-component of the velocity, m/s or --}
\nomenclature[aW]{$W$}{cross-sectional width of inlet and outlet sections, m}
\nomenclature[aWc]{$W_{\text{c}}$}{cross-sectional width of contraction section, m}
\nomenclature[ax]{$x$}{streamwise coordinate, --}
\nomenclature[ay]{$y$}{transverse coordinate, --}
\nomenclature[aY]{$Y$}{electroviscous correction factor (\eqns\ref{eq:27}, and \ref{eq:40}), --}
\nomenclature[azj]{$z_{j}$}{valency of the ions of type j, assumed equal ($z_{+}=\rev{-}z_{-}=z$), --}
%
%------- {Greek symbols}
%
\nomenclature[gdP]{$\Delta P$}{pressure drop (\eqns\ref{eq:38}), --}
\nomenclature[geps0]{$\varepsilon_{\text{0}}$}{permittivity of free space (i.e. vaccum), F/m or C/(V.m)}
\nomenclature[gepsr]{$\varepsilon_{\text{r}}$}{dielectric constant (absolute or relative permittivity) of the electrolyte liquid, --}
%\nomenclature[glambdad]{$\lambda_{\text{D}}$}{Debye length, $\left(=\sqrt{\frac{\varepsilon_{\text{0}}\varepsilon_{\text{r}} k_{\text{b}}T}{z^2e^2n_{\text{0}}}}\right)$, m}
\nomenclature[glambdad]{$\lambda_{\text{D}}$}{Debye length ($=K^{-1}$), \del{m} \rev{--}}
\nomenclature[gmu]{$\mu$}{viscosity, Pa.s}
\nomenclature[gmueff]{$\mu_\text{eff}$}{effective or apparent viscosity, Pa.s}
\nomenclature[gpsi]{$\psi$}{EDL potential (\eqn\ref{eq:2a}), V or --}
\nomenclature[grho]{$\rho$}{density of fluid, kg/m$^3$}
\nomenclature[grhoe]{$\rho_{\text{e}}$}{charge density of liquid, C/m$^3$}
\nomenclature[gsigmab]{$\sigma_\text{\del{b}\rev{i}}$\del{, $\sigma_\text{t}$}}{surface charge density, C/m$^2$}
%\nomenclature[gsigmae]{$\sigma_{\text{e}}$}{electrical conductivity of an electrolyte solution (\eqn\ref{eq:16}), A/(V.m)}
%\nomenclature[gsigma]{$\sigma_\text{t}$}{top wall surface charge density, C/m$^2$}
%
%------- {Dimensionless group}
%
\nomenclature[dbeta]{$\mathit{\beta}$}{liquid parameter (\eqn\ref{eq:1}), --}
\nomenclature[dK]{$\mathit{K}$}{inverse Debye length (\eqn\ref{eq:1}), --}
\nomenclature[dPe]{$Pe$}{Peclet number ($={Re}\times\mathit{Sc}$) (\eqn\ref{eq:1}), --}
\nomenclature[dRe]{$Re$}{Reynolds number (\eqn\ref{eq:1}), --}
\nomenclature[dSa]{$\mathit{S_\text{b}}$, $\mathit{S_\text{t}}$}{surface charge density (\eqn\ref{eq:12}), --}
\nomenclature[dSc]{$\mathit{Sc}$}{Schmidt number (\eqn\ref{eq:1}), --}
\nomenclature[dSb]{$\mathit{S_\text{r}}$}{surface charge density ratio (\eqn\ref{eq:12}), --}
%\nomenclature[dSt]{$\mathit{S_\text{t}}$}{top wall surface charge density (\eqn\ref{eq:12}), --}
%
%%%%%%%%%%% subscripts and superscripts
\nomenclature[sz]{$0$}{without electroviscous effects}
%\nomenclature[szz]{$00$}{without electroviscous and slip effects}
\nomenclature[sc]{$c$}{contraction}
\nomenclature[sd]{$d$}{downstream}
\nomenclature[se]{$e$}{extra or excess}
\nomenclature[sf]{$evac$}{electroviscous and asymmetric charge}
\nomenclature[sm]{$m$}{mathematical}
\nomenclature[ss]{$s$}{statistical}
\nomenclature[su]{$u$}{upstream}
%\nomenclature[sN]{$N$}{normalized values}
%
%\printnomenclature



